FAIR-Pruner: A Flexible Framework for Automatic Layer-Wise Pruning via Tolerance of Difference

Structured pruning is a standard tool for compressing deep neural networks, but its practical performance depends on how sparsity is allocated across layers. We propose FAIR-Pruner, a search-free framework for adaptive layer-wise structured pruning. FAIR-Pruner uses two within-layer rankings: a removal-oriented signal that proposes candidate units and a protection-oriented signal that identifies task-sensitive units. Its core component, Tolerance of Difference (ToD), measures the overlap between the removal prefix and the protected tail, and uses a shared tolerance level to induce non-uniform pruning depths across layers. As a default vision instantiation, FAIR-Pruner combines a Wasserstein-based U-Score for class-conditional unit separability with a Taylor-based R-Score for task-level sensitivity; the same ToD allocation rule can also be paired with alternative removal signals. Theoretically, we analyze ToD through the population R-Score, derive rank-based control of the high-R-Score mass entering the pruning set, and identify an additive exchange condition for same-budget comparison with uniform pruning. Experiments on CIFAR-10, CIFAR-100, SVHN, and ImageNet across VGG, ResNet, DenseNet, ConvNeXt, and DeiT show strong accuracy--compression trade-offs. Prune-only experiments on routed-expert Qwen1.5-MoE-A2.7B-Chat further examine architectural extensibility under matched expert budgets. FAIR-Pruner is released as a pip-installable open-source package.

==> table/DeiT-BandConvNext.before_hongrong_style_polish.tex <==
\begin{table*}[t]
\centering
\caption{Comparison on modern block-structured architectures. 
Unlike the classical CNN benchmarks in Table~\ref{tab:sota_all}, these experiments prune structured components inside modern blocks. 
For ConvNeXt, the pruned components are MLP hidden dimensions inside convolutional blocks; for DeiT-B, the pruned components include attention heads and MLP hidden dimensions. 
FLOPs are reported in GFLOPs. FAIR-Pruner rows are highlighted by the method name for readability.}
\label{tab:modern_architectures}
\setlength{\tabcolsep}{3.5pt}
\small
\begin{tabular}{lllcccc}
\hline
Benchmark / Model & Pruned components & Method 
& Top-1 (\%) & $\Delta$ Top-1 (pp) & GFLOPs & $\Delta$ FLOPs $\downarrow$ \\
\hline

\multirow{6}{*}{CIFAR-100 / ConvNeXt}
& \multirow{6}{*}{MLP hidden}
& Baseline (Unpruned) & 90.01 & --    & 8.683 & -- \\
& & MetaPruning~\cite{liu2019metapruning}       & 82.61 & -7.40  & 3.275 & 62.3\% \\
& & Li et al.~\cite{li2017pruning}              & 68.07 & -21.94 & 3.499 & 59.7\% \\
& & Taylor~\cite{molchanov2019importance}       & 83.36 & -6.65  & 2.328 & 73.2\% \\
& & FPGM~\cite{he2019filter}                    & 80.76 & -9.25  & 2.358 & 72.8\% \\
& & \textbf{FAIR-Pruner (Ours)}                 & 82.96 & -7.05  & 2.391 & 72.5\% \\
\hline

\multirow{5}{*}{ImageNet-1K / DeiT-B}
& \multirow{5}{*}{Attention heads + MLP}
& Baseline~\cite{touvron2021training}           & 81.80 & --     & 16.8 & -- \\
& & WDPruning~\cite{yu2022width}                 & 80.76 & -1.04  & 9.9  & 41.1\% \\
& & IA-RED~\cite{pan2024interpretability}        & 80.30 & -1.50  & 11.8 & 29.8\% \\
& & ITPruner~\cite{zheng2025information}         & 81.20 & -0.60  & 9.9  & 41.1\% \\
& & \textbf{FAIR-Pruner (Ours)}                  & 81.20 & -0.60  & 9.9  & 41.1\% \\
\hline
\end{tabular}
\end{table*}

==> table/DeiT-BandConvNext.before_pruned_component_clarification.tex <==
\begin{table*}[t]
\centering
\caption{Comparison on modern block-structured architectures. 
Unlike the classical CNN benchmarks in Table~\ref{tab:sota_all}, these experiments prune structured components inside modern blocks. 
For ConvNeXt, the pruned components are MLP hidden dimensions inside convolutional blocks; for DeiT-B, the pruned components include attention heads and MLP hidden dimensions. 
FLOPs are reported in GFLOPs. The ConvNeXt competitor rows are reproduced in our unified setting; the DeiT-B competitor rows are taken from the cited papers. FAIR-Pruner rows are highlighted by the method name for readability.}
\label{tab:modern_architectures}
\setlength{\tabcolsep}{3.5pt}
\small
\begin{tabular}{lllcccc}
\hline
Benchmark / Model & Pruned components & Method 
& Top-1 (\%) & $\Delta$ Top-1 (pp) & GFLOPs & $\Delta$ FLOPs $\downarrow$ \\
\hline

\multirow{6}{*}{CIFAR-100 / ConvNeXt}
& \multirow{6}{*}{MLP hidden}
& Baseline (Unpruned) & 90.01 & --    & 8.683 & -- \\
& & MetaPruning~\cite{liu2019metapruning}       & 82.61 & -7.40  & 3.275 & 62.3\% \\
& & Li et al.~\cite{li2017pruning}              & 68.07 & -21.94 & 3.499 & 59.7\% \\
& & Taylor~\cite{molchanov2019importance}       & 83.36 & -6.65  & 2.328 & 73.2\% \\
& & FPGM~\cite{he2019filter}                    & 80.76 & -9.25  & 2.358 & 72.8\% \\
& & \textbf{FAIR-Pruner (Ours)}                 & 82.96 & -7.05  & 2.391 & 72.5\% \\
\hline

\multirow{5}{*}{ImageNet-1K / DeiT-B}
& \multirow{5}{*}{Attention heads + MLP}
& Baseline~\cite{touvron2021training}           & 81.80 & --     & 16.8 & -- \\
& & WDPruning~\cite{yu2022width}                 & 80.76 & -1.04  & 9.9  & 41.1\% \\
& & IA-RED~\cite{pan2024interpretability}        & 80.30 & -1.50  & 11.8 & 29.8\% \\
& & ITPruner~\cite{zheng2025information}         & 81.20 & -0.60  & 9.9  & 41.1\% \\
& & \textbf{FAIR-Pruner (Ours)}                  & 81.20 & -0.60  & 9.9  & 41.1\% \\
\hline
\end{tabular}
\end{table*}


==> table/ImageNet_SOTA_ResNet-50.tex <==
\begin{table}\caption{Comparison of structured pruning methods on ImageNet-1K with ResNet-50~\citep{he2016deep} in terms of Top-1 accuracy and computational cost. The best-performing result is shown in bold. Methods marked with $^*$ use additional techniques such as knowledge distillation, expanded search spaces, or extra training tricks.}
\setlength{\tabcolsep}{2.5mm}
\centering
\begin{tabular}{c c c c}
\hline
Method & Top-1 (\%) & MFLOPs & $\Delta\text{FLOPs}\downarrow$ \\ 
\hline
% \multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}ResNet-56\\ \cite{he2016deep}\end{tabular}} 
  Baseline(Unpruned) & 76.88 & 4089&-\\
  GAL~\citep{lin2019towards}  &71.95 & 2330 &43.0\% \\ 
  Metapruning$^*$ \cite{liu2019metapruning}  & 72.17  & 2260 & 44.7\%\\
  Random Pruning~\citep{li2022revisiting}  & 75.13  & 2074 &49.3\% \\ 
  HRank~\citep{lin2020hrank} & 74.98 & 2300 &43.8\%\\ 
  DECODER-6~\citep{alwani2022decore} & 74.58 & 2372 &42.0\%\\ 
  ITPruner~\citep{zheng2025information}  & 75.28  & 1943 &52.5\% \\ 
  MFP~\citep{he2019filter}  & 74.86 & 1942 &52.5\% \\ 
  \textbf{FAIR-Pruner (Ours)} & \textbf{75.29} &  \textbf{1932} &52.8\% \\ 
\hline
% \multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}DenseNet-40\\ \cite{huang2017densely}\end{tabular}} 
  
\hline
\end{tabular}

\label{table:resnet50_comparison}
\end{table}


